Compressed Sensing MRI Reconstruction using a Generative Adversarial Network with a Cyclic Loss

Compressed Sensing MRI (CS-MRI) has provided theoretical foundations upon which the time-consuming MRI acquisition process can be accelerated. However, it primarily relies on iterative numerical solvers which still hinders their adaptation in time-critical applications. In addition, recent advances in deep neural networks have shown their potential in computer vision and image processing, but their adaptation to MRI reconstruction is still in an early stage. In this paper, we propose a novel deep learning-based generative adversarial model, RefineGAN, for fast and accurate CS-MRI reconstruction. The proposed model is a variant of fully-residual convolutional autoencoder and generative adversarial networks (GANs), specifically designed for CS-MRI formulation; it employs deeper generator and discriminator networks with cyclic data consistency loss for faithful interpolation in the given under-sampled k-space data. In addition, our solution leverages a chained network to further enhance the reconstruction quality. RefineGAN is fast and accurate -- the reconstruction process is extremely rapid, as low as tens of milliseconds for reconstruction of a 256x256 image, because it is one-way deployment on a feed-forward network, and the image quality is superior even for extremely low sampling rate (as low as 10%) due to the data-driven nature of the method. We demonstrate that RefineGAN outperforms the state-of-the-art CS-MRI methods by a large margin in terms of both running time and image quality via evaluation using several open-source MRI databases.

==> background.tex <==
% !TEX root = main.tex


\begin{figure*}[ht!]
	\centering
	\includegraphics[width=1\textwidth]{overview/ReconGAN_Overview.pdf}
	\caption{Overview of the proposed method: it aims to reconstruct the images which are satisfied the constraint of under-sampled measurement data; and whether those look similar to the fully aliasing-free results. Additionally, if the fully sampled images taken from the database go through the same process of under-sampling acceleration; we can still receive the reconstruction as expected to the original images.}
	\label{fig:overview}	
\end{figure*}



\label{sec:background}
%\del{
In this section, we will briefly overview the basics of Compressed Sensing MRI.
%
\stkout{In the following discussion, we use the subscript $f$ to denote the result of applying a masked Fourier transform to a given variable.}
%
\rv{We denote the under-sampled raw MRI data ($k$-space measurements) using the sampling mask $R$ as $m$. }% that we wish to reconstruct as $m$.
%
\rv{Then, its zero-filling reconstruction $s_0$ can be obtained by the following equation:
\begin{equation}
s_0 = {F^H}{R^H}\left( {{m}} \right)
\end{equation}
where $F$ is the Fourier operator, and superscript $H$ indicates the conjugated transpose of a given operator. 
%
%Intuitively, turning any image $s$ into under-sampled measurement $m$ can be done via the inverse of the reconstruction process: 
Similarly, turning any image $s_i$ into its under-sampled measurement $m_{s_i}$ with the given sampling mask $R$ can be done via the inverse of the reconstruction process: 
%
\begin{equation}
{m_{s_i}} = RF\left( s_i \right)
\end{equation}
%}
}
%
%
%
%\rv{
%In the following discussion, we use the subscript $f$ to denote the result of applying a masked Fourier transform to a given variable. 
%}
%\subsection{Overview of Compressed Sensing MRI}
%
\rv{
Then, compressed sensing MRI reconstruction, which is a process of generating a full-reconstruction image $s$ from under-sampled $k$-space data $m$, can be described as follows:
\begin{equation}
\mathop {\min }\limits_s  {J}\left( {s} \right)\quad s.t.\quad {RF(s)} = {m}\
\end{equation}
}
\stkout{where $F$ is the Fourier operator, $R$ is the sampling mask, and superscript $H$ indicates the conjugated transpose of a given operator.
%
and the above constrained problem can be reformulated in an unconstrained fashion with weighting parameters as follows:
%
}
%\stkout{
\begin{equation}
\stkout{
\mathop {\min }\limits_s \left\| {{RF(s)} - {m}} \right\|_2^2 + \lambda J\left( s \right)\quad
}
\end{equation}
%}
\rv{
where ${J\left( s \right)}$ is a regularizer required for ill-posed optimization problems.
%
In our method, this energy minimization process is replaced by the training process of the neural network.}

%
%Solving such this ill-posed problem involves some types of regularization to choose the best among candidate solutions. 
%Without the support of the regularizer ${J\left( s \right)}$, it is difficult to choose among the candidate solutions since reconstructing the image from the constraint of data consistency only, by itself, is an ill-posed problem. 
%
\stkout{ 
Many classical priors can be used for ${J\left( s \right)}$, such as Tikhonov regularization (IID Gaussian prior)~\cite{chaari2008autocalibrated}, edge-preserving regularization~\cite{tian2011low}, total variation (TV)~\cite{chen2013calibrationless}, non-local mean filter (NLM)~\cite{manjon2008mri}, wavelets~\cite{pizurica2006review}, curvelets~\cite{bhadauria2013medical}, etc. 
%
By enforcing $\ell_p$ norm where $0\leq p \leq 1$ for regularization, compressed sensing theory~\cite{donoho2006compressed, candes2008introduction} can be applied to MRI reconstruction from highly undersampled $k$-space data~\cite{lustig2008compressed}. 
%
This sparsity-induced image reconstruction method aims to find the solution (images $s$) that satisfies not only the under-sampled measurement constraints but also sparsity in the transformed domain by decomposing the signals with the designated universal transform sparsity basis. 
% 
For example, the seminal work by Lustig \textit{et al.}~\cite{MRM:MRM21391} proposed that ${J\left( s \right)}$ is equal to $ {\left\| {\Psi s} \right\|_0}$, in which $\Psi$ is the wavelet transform, and further relaxed the $\ell_0$ norm by $\ell_1$ norm substitution. 
}
%%
%Solving such nonlinear optimization problems usually involves an iterative process to minimize the data consistency energy and the sparsity energy.
%%
%Therefore, the primary goal of the present work is leveraging state-of-the-art deep learning for modeling $\ell_1$-regularized CS-MRI formulations to avoid the time-consuming iterative optimization process as well as to improve the quality of the reconstructed image. 









==> discussion.tex <==
\label{sec:discussion}
